Ordered Graph Limits and Their Applications

The emerging theory of graph limits exhibits an analytic perspective on graphs, showing that many important concepts and tools in graph theory and its applications can be described more naturally (and sometimes proved more easily) in analytic language. We extend the theory of graph limits to the ordered setting, presenting a limit object for dense vertex-ordered graphs, which we call an orderon. As a special case, this yields limit objects for matrices whose rows and columns are ordered, and for dynamic graphs that expand (via vertex insertions) over time. Along the way, we devise an ordered locality-preserving variant of the cut distance between ordered graphs, showing that two graphs are close with respect to this distance if and only if they are similar in terms of their ordered subgraph frequencies. We show that the space of orderons is compact with respect to this distance notion, which is key to a successful analysis of combinatorial objects through their limits. We derive several applications of the ordered limit theory in extremal combinatorics, sampling, and property testing in ordered graphs. In particular, we prove a new ordered analogue of the well-known result by Alon and Stav [RS\&A'08] on the furthest graph from a hereditary property; this is the first known result of this type in the ordered setting. Unlike the unordered regime, here the random graph model $G(n, p)$ with an ordering over the vertices is not always asymptotically the furthest from the property for some $p$. However, using our ordered limit theory, we show that random graphs generated by a stochastic block model, where the blocks are consecutive in the vertex ordering, are (approximately) the furthest. Additionally, we describe an alternative analytic proof of the ordered graph removal lemma [Alon et al., FOCS'17].

==> AlonStav.tex <==
\newcommand{\balpha}{{\boldsymbol{\alpha}} }

 \section{The furthest ordered graph from a hereditary property}\label{sec:furthest}
%\red{Omri: Need to define ``flexible'' somewhere sooner.}

In this section we prove Theorem~\ref{thm:ordered_Alon_Stav}. The proof roughly follows along the same lines as the proof of Lov\'asz and Szegedy for the
unordered setting~\cite{LS10}. However, before proceeding, let us show why an exact analogue of Theorem~\ref{thm:Alon-Stav-unordered} cannot hold for the ordered setting.

\subsection{The random graph $\bG(n,p)$ is not always the furthest}
\label{subsec:furthest_tehnical}
Recall the hereditary property $\calH$ defined in Subsection~\ref{subsec:furthest_intro}. For convenience, let us describe $\calH$ again. An ordered graph $G$ satisfies $\calH$ if and only if there do not exist vertices $u_1 < u_2 \leq u_3 < u_4$ in $G$ where $u_1 u_2$ is a non-edge and $u_3 u_4$ is an edge.
Here we prove that (a direct analogue of) Theorem~\ref{thm:Alon-Stav-unordered} does not hold for $\calH$, that is, for any $p$, a typical graph $G \sim G(n,p)$ is \emph{not} asymptotically the furthest graph from $\calH$. We contrast this by describing, for any $n \in \mathbb{N}$, a graph $G$ on $n$ vertices that \emph{is} the furthest from $\calH$ up to an $o(1)$ term.

The following lemma characterizes the property $\calH$ in a way that will make it fairly straightforward, given an ordered graph $G$, to estimate the distance $d_1(G, \calH)$.
\begin{lemma}[Thresholding lemma]\label{lem:threshold_hered_property}
	An ordered graph $G$ on vertices $v_1 < v_2 < \cdots < v_n$ satisfies $\calH$ if and only if there exists a ``threshold'' $i \in [n]$ for which the following two conditions hold.
	\begin{itemize}
		\item For any $1 \leq j < j' \leq i$, the vertices $v_j$ and $v_{j'}$ are \emph{connected} in $G$.
		\item For any $i+1 \leq j < j' \leq n$, the vertices $v_j$ and $v_{j'}$ are \emph{not connected} in $G$.
	\end{itemize}
\end{lemma}
%The proof of the lemma is simple and elementary; for readability purposes, it is relegated to Section \ref{sec:furthest}.
\begin{proof}
	Suppose first that $G \in \calH$, and pick the maximal $i \in [n-1]$ for which all pairs of the form $v_jv_{j'}$ where $1 \leq j < j' \leq i$ are connected in $G$. The first condition holds trivially, and it only remains to prove the second one. Suppose on the contrary that it does not hold, which means that $i < n-1$ and that $v_j$ and $v_{j'}$ are connected for some $i+1 \leq j < j' \leq n$. By the maximality of $i$, there exists some $j'' \leq i$ for which $v_{j''}v_{i+1}$ is \emph{not} an edge. Since $i+1 \leq j$, the four vertices $v_{j''} < v_{i+1} \leq v_j < v_{j'}$ induce the ordered pattern forbidden by $\calH$, a contradiction.

	Conversely, if there exists $i$ for which the two conditions hold, then for any tuple of vertices $v_{j_1}, v_{j_2}, v_{j_3}, v_{j_4}$ where $j_1 < j_2 \leq j_3 < j_4$, at least one of the following holds. Either we have $j_2 \leq i$, meaning that $v_{j_1} v_{j_2}$ is an edge, or $j_3 \geq i+1$, meaning that $v_{j_3} v_{j_4}$ is a non-edge. In both cases, the tuple does not violate the condition in the definition of $\calH$.
\end{proof}

Using Lemma~\ref{lem:threshold_hered_property}, we can estimate the typical distance of a graph $G \sim \bG(n,p)$ from $\calH$.
\begin{lemma}
	For any $n \in \mathbb{N}$ and $p \in [0,1]$ (possibly depending on $n$), a graph $G \sim \bG(n,p)$ satisfies with high probability that $d_1(G, \calH) = p(1-p) + o(1) \leq \frac{1}{4} + o(1)$.
\end{lemma}
\begin{proof}
	Standard Chernoff-type concentration bounds show that w.h.p.~the following holds for all $i \in [n]$: the number of non-edges among the first $i$ vertices is $(1-p)i^2/2 + o(n^2)$, and the number of edges among the last $n-i$ vertices is $p(n-i)^2/2 + o(n^2)$. Thus, w.h.p.~we have
	\begin{equation}
	\label{eq:dist_of_random_graph}
	d_1(G, \calH) = \frac{1}{\binom{n}{2}} \min_{i \in [n]} \left( (1-p)\frac{i^2}{2} + p\frac{(n-i)^2}{2} + o(n^2)  \right) = p(1-p) + o(1)
	\end{equation}
	where the minimum of the sum (up to the $o(n^2)$ term) is attained for $i \in \{\lfloor np \rfloor, \lceil np \rceil\}$. The $p(1-p)$ term is maximized at $p = 1/2$, where it equals $1/4$. %In other words, the maximal distance that we can hope to get by taking $G \sim \bG(n,p)$ is $1/4 + o(1)$, attained at $p = 1/2$.
\end{proof}

On the other hand, there exist large graphs whose distance from $\calH$ is much larger than $1/4$.
\begin{lemma}
	Let $n \in \mathbb{N}$, and consider the graph $G$ on the vertex set $[n]$ with the standard ordering, where $u$ and $v$ are connected if and only if $u+v \geq n$. The graph $G$ satisfies $d_1(G, \calH) \geq 1/2 - o(1)$.
\end{lemma}
\begin{proof}
	Fix any $i \in [n]$. Without loss of generality, we may assume that $i \leq n/2$ (the case $i > n/2$ is symmetric).
	On one hand, the number of non-edges between pairs of vertices $j < j' \in [i]$ is $\binom{i}{2}$. On the other hand, a straightforward calculation shows that the number of edges between pairs of vertices $j,j'$ where $i+1 \leq j < j'$ is $\frac{1}{2}\binom{n}{2} - \binom{i}{2} - o(n^2)$. Thus, the number of edges that one needs to add or remove if the threshold of Lemma~\ref{lem:threshold_hered_property} is set to $i$ is $\frac{1}{2}\binom{n}{2} - o(n^2)$ (regardless of the value of $i$), implying that $d_1(G, \calH) \geq 1/2 - o(1)$.
\end{proof}

Conversely, it is trivial that $\overline{d_\calH} \leq 1/2$, as any graph $G$ can be turned into either a complete or empty graph (which both satisfy $\calH$) by adding or removing at most $\frac{1}{2}\binom{n}{2}$ edges. Combined with the last lemma, we conclude that $\overline{d_{\calH}} = 1/2$.

\subsection{Proof of Theorem~\ref{thm:ordered_Alon_Stav}}
\label{subsec:furthest-proof}
We continue to the proof of Theorem~\ref{thm:ordered_Alon_Stav}.
To begin, we first establish several basic properties of hereditary properties in the ordered setting, starting with a discussion on their \emph{closure} in the space of orderons.

Let $\calH$ be a hereditary ordered graph property ($\calH$ will be fixed throughout the section). Recall that a property is \emph{hereditary} if it satisfies the following: if $G\in\calH$ then every induced subgraph of $G$ (vertex repetitions are not allowed) is also in $\calH$.

In general, we define the \emph{closure} $\barP$ of an ordered graph property $\calP$ as the set of all orderons $W$ for which there exists a sequence of graphs $G_n \in \calP$ (with $|V(G_n)| \to \infty$) that converges to $\calP$ in $d_{\triangle}$. Note that $\barP$ is a closed set in $\calW$ with respect to $d_{\triangle}$ (also note that it is generally \emph{not} true that $W_G \in \barP$ for any $G \in \calP$). The following characterization for the closure of a hereditary property will be useful in multiple occasions along this section as well as in Section \ref{sec:hereditary}.

\begin{lemma}\label{lem:conditions_closure}
	Let $\calH$ be a hereditary property of ordered graphs. The following conditions are equivalent for an orderon $W$.
	\begin{itemize}
		\item $W \in \barH$.
		\item $t(F,W) = 0$ for any ordered graph $F \notin \calH$.
		\item $\Prx[\bG(k,W)\in \calH]=1$ for every $k$.
	\end{itemize}
\end{lemma}
\begin{proof}
	The second and third conditions are clearly equivalent: for any fixed $k$, the probability that $\bG(k,W)\notin \calH$ is the sum of $t(F, W)$ over all $F \notin \calH$ on $k$ vertices. We now show equivalence between the first condition and the other two. If $W \in \barH$ then there exists a sequence of ordered graphs $G_n \in \calH$ with $|V(G_n)| \to \infty$ that converges to $W$ in $d_{\triangle}$. Fix $k$. For any $n$, the density $t(F, W_n)$ is bounded by the probability that, when picking $k$ vertices from a set of $n$ vertices with repetition, some vertex will be picked more than once (see Observation \ref{Obs:GraphsToOrderons} for more details). This probability is bounded by $\binom{k}{2}/n \to 0$, that is, $t(F, W_n) \to 0$ as $n \to \infty$.
	Since $G_n \to W$, it follows that $t(F, W) = \lim t(F, W_n) = 0$. The converse follows immediately from the third condition combined with our sampling theorem, which together show that with high probability, a large enough sample of $W$ will both satisfy $\calH$ and be arbitrarily close to $W$ in $d_{\triangle}$.
\end{proof}

We will need the definition of a \emph{flexible} property, given below; this is an ordered analogue of flexible properties in the unordered setting, defined in \cite{LS10}.

\begin{definition}[support, flexibility]
	For an orderon $W \in \calW$ and a value $0 \leq \alpha \leq 1$, the $\alpha$-support of $W$, denoted $\supp_\alpha(W)$, is the set of all pairs $(u,w) \in ([0,1]^2)^2$ for which $W(u,v) = \alpha$.

	We say that a property $\calR$ is \emph{flexible} if for any $W, W' \in \calW$ where $\supp_\alpha(W) \subseteq \supp_\alpha(W')$ for $\alpha = 0,1$ and $W \in  \calR$ it holds that $W' \in \calR$ as well. In particular, this means that the supports $\supp_{\alpha}(W)$ for $\alpha = 0,1$ fully determine whether $W$ satisfies a given flexible property.
\end{definition}

%\begin{definition}[flexing, flexible property]
%	For two orderons $U, W \in \calW$, we say that $U$ is a \emph{flexing} of $W$ if $U(u,v) = W(u,v)$ for any $(u,v) \in ([0,1]^2)^2$ satisfying that $W(u,v) \in \{0,1\}$.
%
%	A property $\calP$ of orderons is \emph{flexible} if the flexing of any orderon $W \in \calP$ is also in $\calP$.
%\end{definition}


\begin{lemma}\label{lem:U-flexing} The closure $\barH$ of a hereditary property is flexible.
\end{lemma}
\begin{proof}
	By Lemma~\ref{lem:conditions_closure}, the closure of a hereditary property can be defined by conditions of the form $t(F,U)=0$ (for all graphs $F\notin \calH$). For every fixed $F\notin \calH$, this condition means that for almost all vectors $v\in [0,1]^{|V(F)|}$, at least one of the factors in
	$\prod_{{(i,j)\in E_{<}}}U(v_i,v_j)\cdot\prod_{{(i,j)\in \overline{E}_{<}}}(1-U(v_i,v_j))$
	must be $0$. This condition is preserved if values of $W$ that are \emph{strictly} between $0$ and $1$ are changed to any other value (including $0$ and $1$).
\end{proof}


The next lemma shows, using the flexibility, that the distance from the closure of a hereditary property is a concave function over the space of orderons.

\begin{lemma}\label{lem:distance_is_concave}
	Let $\calH$ be a hereditary ordered graph property.
	The distance $d_1(\cdot, \barH)$ is a concave function over $\calW$.
\end{lemma}
\begin{proof}
	Let $W_1, W_2, U \in \calW$ be three orderons satisfying $U = \lambda W_1 + (1-\lambda) W_2$ for some $0 < \lambda < 1$. It suffices to show that $d_1(U, \barH) \geq \lambda d_1(W_1, \barH) + (1-\lambda)d_1(W_2, \barH)$. The crucial observation is that $\supp_\alpha(U) = \supp_\alpha(W_1) \cap \supp_\alpha(W_2)$ for $\alpha = 0, 1$.

	Let $U'$ be any orderon in $\barH$. We show that there exist $W'_1, W'_2 \in \barH$ so that $$\lambda d_1(W_1, W'_1) + (1-\lambda) d_1(W_2, W'_2) \leq d_1(U, U').$$
	Indeed, for $i = 1,2$ pick $W'_i$ as the unique orderon satisfying the following: $W'_i(u,v) = 0$ for $(u,v) \in \supp_0(U')$; % \setminus \supp_0(U)$;
	$W'_i(u,v) = 1$ for $(u,v) \in \supp_1(U')$; % \setminus \supp_1(U)$;
	and otherwise, $W'_i(u,v) = W_i(u,v)$. By Lemma~\ref{lem:U-flexing}, $W'_1, W'_2 \in \barH$, and it is easy to verify that $W'_1, W'_2$ satisfy the desired inequality. The proof of the lemma now follows by taking the infimum over all $U',W_1',W_2'\in \calH$.
\end{proof}


%\begin{proof}
%Let $W,W',U \in \calW$ be three orderons where $U = \lambda W + (1-\lambda) W'$ for some $0 < \lambda < 1$. Fix $\varepsilon > 0$ and let $Z,Z' \in \calR$ be orderons that satisfy $d_1(W, Z) \leq d_1(W, \calR) + \varepsilon$ and $d_1(W', Z') \leq d_1(W', \calR) + \varepsilon$ and note that
%\end{proof}

Recall that an orderon $W$ is called \emph{naive} if its values do not depend on the second (``variability'') coordinate. That is, for every $x,y\in[0,1] $ it holds that $W((x,a), (y,b)) = W((x, a'), (y, b'))$ for any $a,a',b,b' \in [0,1]$.
Our next goal is to show, using the concavity, that for any hereditary property $\calH$ and orderon $W$ there exists a naive orderon $W'$ at least as far from $\barH$ as $W$.



\begin{lemma}
	For any hereditary property $\calH$ and orderon $W$ there exists a naive orderon $W'$ so that $d_1(W', \barH) \geq d_1(W, \barH)$.
\end{lemma}

\begin{proof}
	To prove the lemma, we combine the concavity guaranteed by the previous lemma with some measure-theoretic and probabilistic tools.
	For any $(x,y) \in [0,1]^2$ define $\mu^{x,y}$ as the expectation, over all $(a,b) \in [0,1]^2$, of $W((x,a), (y,b))$. We will prove that the unique $W' \colon ([0,1]^2)^2 \to [0,1]$ for which $W'((x,a),(y,b)) = \mu^{x,y}$ for all $(x,y)$ satisfies the conditions of the lemma. (To show that $W'$ is a naive orderon one needs to prove that $W'$ as defined above is indeed a measurable function, but this will follow from the proof.)
	%Specifically, we show that for any integer $n \leq 2$, there exists an orderon $W_n$ satisfying the following conditions.
	%\begin{itemize}
	%	\item $d_1(W_n, \barH) \geq d_1(W, \barH)$.
	%	\item There exists $A_n \subseteq [0,1]^2$ of measure $1-1/n^2$, so that $W_n$ is ``naive when restricted to $A_n$'', namely, $W_n((x, a), (y, b)) = W_n((x, a'), (y, b'))$ for any $(a,b,a',b') \in [0,1]^4$.
	%\end{itemize}
	%We conclude by showing that $W_n \to W'$ where the convergence is even pointwise, and deduce that $d_1(W', \barH) \geq d_1(W, \barH)$.

	Fix an integer $n$ and pick $A_n = \{(x,y) \in [0,1]^2 : Q_n(x) \neq Q_n(y) \}$, where the function $Q_n$ is as defined in the beginning of Section~\ref{sec:block_orderons}.
	Consider the family of measure-preserving bijections $f_{\alpha_1, \alpha_2, \ldots, \alpha_n}$, where $(\alpha_1, \ldots, \alpha_n) \in [0,1]^n$, defined as follows: For any $(x,a) \in [0,1]^2$, we set $f_{\alpha_1, \alpha_2, \ldots, \alpha_n}(x,a) = (x, a+\alpha_{Q_n(x)})$. Note that $\shift{f_{\alpha_1, \alpha_2, \ldots, \alpha_n}} = 0$ always holds. As these bijections clearly do not change the $L^1$-distance of $W$ from $\barH$, we have that $d_1(W, \barH) = d_1(W^{f_{\alpha_1, \alpha_2, \ldots, \alpha_n}}, \barH)$ for any choice of $(\alpha_1, \ldots, \alpha_n) \in [0,1]^n$.

	Pick $n$ tuples $\{(\balpha^i_1, \ldots, \balpha^i_n)\}_{i=1}^{n}$ uniformly at random. Set $\bg_i = f_{\balpha^i_1, \ldots, \balpha^i_n}$ and consider the orderon
	$$U_n = \frac{1}{n} \sum_{i=1}^{n} W^{\bg_i} = \frac{1}{n} \sum_{i=1}^{n} W^{f_{\balpha^i_1, \ldots, \balpha^i_n}}.$$
	Since each $\bg_i$ is a measure-preserving bijection with shift zero, we have that $d_1(W, \barH) = d_1(W^{\bg_i}, \barH)$. As $U_n$ is a convex combination of the $W^{\bg_i}$, we get that
	$$
	d_1(U_n, \barH) \geq \frac{1}{n} \sum_{i=1}^{n} d_1(W^{\bg_i}, \barH) = d_1(W, \barH).
	$$

	Now, given any fixed orderon $U \in \{U_n, W^{\bg_1}, W^{\bg_2}, \ldots, W^{\bg_n}\}$ and $(x,y) \in [0,1]^2$, define the random variable $\bX_U^{x,y}$ as follows: pick $(\ba,\bb) \in [0,1]^2$ uniformly at random, and return the value $U((x,\ba), (y,\bb)) - \mu^{x,y}$. Note that the expectation of $\bX_U^{x,y}$ for any $U$ as above is zero.

	A basic probabilistic fact states that, for $n$ i.i.d.\ bounded random variables $\bY_1, \ldots, \bY_n$, the variance of $\ol{ \bY }= (\bY_1 + \cdots + \bY_n) / n$ equals $\Var(\bY_1) / n$, and tends to zero as $n \to \infty$. Fix some $(x,y) \in A_n$, and for any $i \in [n]$ take $\bY_i = \bX_{W^{\bg_i}}^{x,y}$. Finally pick $\ol{ \bY} = \bX_{U_n}^{x,y}$, and note that the $\bY_i$ are indeed i.i.d., that $|\bY_i| \leq 1$ (meaning that $\Var(\bY_i) \leq 1$), and that $\ol{ \bY }= \sum \bY_i / n$. It follows that the variance of $\ol{ \bY }= \bX_{U_n}^{x,y}$ is bounded by $1/n$.

	Consequently, for fixed $(x,y) \in A_n$, the probability (ranging over the choices of $\bg_1, \ldots, \bg_n$ and $\ba,\bb \in [0,1]^2$) that $|U_n((x,\ba), (y,\bb)) - \mu^{x,y}| \geq 1/n^{1/3}$ is bounded by $1/n^{1/3}$. Thus, the expected measure of the collection
	$$B_n \eqdef \{(x,a,y,b) : |U_n((x,a), (y,b)) - \mu^{x,y}| \geq 1/n^{1/3} \}$$
	of ``bad'' $(x,a,y,b)$ tuples is bounded by $1/n^{1/3}$ where the randomness is over the choices of $\bg_1, \ldots, \bg_n$. In particular, there exists such a choice of $U_n$ for which $|B_n| \leq 1/n^{1/3}$; we henceforth fix this choice of $U_n$.

	As $|[0,1]^2 \setminus A_n| = 1/n^2 \to 0$ as $n \to \infty$, and $\int_{A_n }|U_n - U_{n'}| \leq 4 / n^{1/3}$ for $n' > n$, it follows that the sequence $\{U_n\}$ is $L^1$-Cauchy. Thus, it converges in $L^1$ to some limit $U'$, and clearly the set of points $\{(x,y) \in [0,1]^2 : U'(x,y) \neq \mu^{x,y}\}$ is of measure zero. In other words, $U'$ is measurable and equals $W'$ defined above almost everywhere, and thus $W'$ is measurable as well and $U_n \to W'$ in $L^1$. As $d_1(U_n, \barH) \geq d_1(W, \barH)$ for any $n$, the inequality still holds at the limit, that is, $d_1(W', \barH) \geq d_1(W, \barH)$. This concludes the proof.
	%
	%We now wish to claim that $U^n_m \to W_n$ where the convergence is in $L^1[[0,1]^4]$, i.e., that our sequence $\{U^n_m\}_{m=1}^{\infty}$ converges in $L^1$ to an ``almost naive'' orderon. However, we have not yet considered ``intra-block'' pairs $(x,y) \in [0,1]^2$ where $Q_n(x) = Q_n(y)$. An argument very similar to the one discussed above asserts that on expectation, the collection of tuples $(x,a,y,b) \in [0,1]^4$ where $Q_n(x) = Q_n(y)$, and $|U((x,a), (y,b)) - \mu_{x,y,b-a}| \geq o_m(1)$ has measure at most $o_m(1)$, where $\mu_{x,y,c}$ is the expectation, over all pairs $(a,a+c \mod 1) \in [0,1]^2$, of $U((x,a), (y,a+c))$. With probability $1/3$ the measure of ``bad'' $(x,y)$ pairs is at most three times the expectation, and thus there exists $U^n_m$ that satisfies both the ``inter-block'' and ``intra-block'' conditions.
	%
	%Now note that the sequence $\{U^n_m\}$ is $L^1$-Cauchy, and thus it converges to a limit $W_n$, that is, $d_1(U^n_m, W_n) \to 0$. Let us verify that $W_n$ satisfies the two conditions stated in the beginning of the proof. The first condition holds since $d_1(U^n_m, \barH) \geq d_1(W, \barH)$ holds for any $n$, and the $L^1$-convergence asserts that this still holds at the limit, that is, $d_1(W_n, \barH) \geq d_1(W, \barH)$. For the second condition, the measure of ``bad'' tuples $(x,a,y,b)$ in $U^n_m$ converges to zero as $m \to 0$, and thus $W_n((x,a), (y,b)) = \mu^{x,y}$ almost everywhere restricted to $A_n$, and can be ensured to hold everywhere by changing the values of $W_n$ on a measure-zero set.
	%
	%Finally, the sequence $\{W_n\}$ is again $L^1$-Cauchy and thus converges to a limit $W'$. A reasoning similar to that of the last paragraph implies that $W'$ is a naive orderon, and satisfies $d_1(W', \barH) \geq d_1(W, \barH)$, as desired.
\end{proof}

\begin{definition}
	For any hereditary property $\calH$ let $\Delta_{\calH}$ denote the supremum of the distance $d_1(W, \barH)$ among all $W \in \calW$.
\end{definition}
The following is an immediate consequence of the last lemma.
\begin{lemma}\label{lem:far_naive}
	For any hereditary property $\calH$ and $\varepsilon > 0$ there exists a naive orderon $W'$ for which $d_1(W', \barH) \geq \Delta_\calH - \varepsilon$.
\end{lemma}

%Generally, in the rest of this section the orderons with which we will work are naive. Such orderons ``behave'' in a sense like graphons where the order is important.
%, and thus many previous results for graphons

With some abuse of notation, we henceforth view a naive orderon $W$ as a measurable symmetric function from $[0,1]^2$ to $[0,1]$ and for $x,y \in [0,1]$ we denote by $W(x,y)$ the (unique) value of $W((x,a), (y,b))$ for $a,b \in [0,1]$.

Recall the definition of a naive block orderon from Section~\ref{sec:block_orderons} (in particular, the fact that the blocks are \emph{consecutive} in terms of order). The next lemma asserts that there exist naive block orderons with a bounded number of blocks, that are almost the furthest away from $\barH$.

\begin{lemma}\label{lem:naive_block_orderon_far}
	Let $\calH$ be a hereditary property and let $\varepsilon > 0$. There exists a naive block orderon $W$ with at most $M_\calH(\varepsilon)$ blocks so that $d_1(W, \barH) \geq \Delta_\calH - \varepsilon$.
\end{lemma}
\begin{proof}
	The proof relies on a fundamental fact in Lebesgue measure theory, stating that (finite) linear combinations of indicator functions of the form $I = I_{[a_i, b_i] \times [c_i, d_i]}$ are dense in the two-dimensional Lebesgue space $L^1[\mathbb{R}^2]$ (and specifically, in $L^1[[0,1]^2]$).
	Indeed, Theorem 2.4 (ii) in \cite{PrincetonLectures} states that for any function $W$ in $L^1[\mathbb{R}^2]$ and $\delta > 0$ there exists $N = N(W, \varepsilon) \geq 0$ and a step function $T$ of the form
	$$
	T = \sum_{i=1}^{N} \alpha_i \cdot I_{[a_i, b_i] \times [c_i, d_i]},
	$$
	where $\alpha_i \in \mathbb{R}$, so that $d_1(W,T) \leq \delta$.
	In our case, $W$ is a naive orderon, and is thus a symmetric function in $L^1[[0,1]^2]$.
	We note that, while Theorem 2.4 (ii) in~\cite{PrincetonLectures} does not guarantee that the function $T$ approximating $W$ is symmetric, we can easily make $T$ symmetric---and in particular, a naive orderon---by replacing it with $(T + \tilde{T})/2$, where $\tilde{T} = \sum_{i=1}^{N} \alpha_i \cdot I_{[c_i, d_i] \times [a_i, b_i]}$.

	We now describe how to construct a naive block orderon which is $L^1$-close to the above $T$.  Recall the definition of $Q_n$ given in the beginning of Section~\ref{sec:block_orderons}, and for $M \geq 4N / \delta$, consider the following weighted ordered graph $G$ on $M$ vertices. Given $(i,j) \in [M]^2$, if $T$ is constant over all pairs $(x,y) \in [0,1]^2$ for which $Q_M(x) = i$ and $Q_M(y) = j$, then we define $G(i,j)$ to be this constant value (and say that $(i,j)$ is good). Otherwise, $G(i,j)$ is defined arbitrarily.
	The number of pairs $(i,j)$ that are not good is at most $4MN$. Indeed, $(i,j)$ might not be good only if the square $[(i-1)/M, i/M] \times [(j-1)/M, j/M]$ intersects the boundary of $[a_\ell, b_\ell] \times [c_\ell, d_\ell]$ for some $\ell \in [N]$. However, the latter boundary intersects at most $4M$ such squares, and summing over all $\ell \in [N]$ we get the desired bound.

	Now let $U$ be the naive block orderon over $M$ blocks defined by $U(x,y) = G(Q_M(x), Q_M(y))$ for any $(x,y) \in [0,1]^2$. We get that $d_1(U, T) \leq 4MN / M^2 \leq \delta$, where the last inequality holds by our choice of $M$. It thus follows that $d_1(W,U) \leq d_1(W,T) + d_1(U,T) \leq 2\delta$.

	To conclude the proof, let $\calH$ be a hereditary property, let $\varepsilon > 0$, and let $W$ be an arbitrary naive orderon satisfying that $d_1(W, \barH) \geq \Delta_\calH - \varepsilon/3$ (the existence of such a $W$ is guaranteed by Lemma~\ref{lem:far_naive}); specifically we can take such a $W$ that minimizes the quantity $N(W, \varepsilon)$, which was defined in the beginning of the proof. Now take $\delta = \varepsilon/3$ and let $U$ denote the naive block orderon over $M = \lceil 4N / \delta \rceil$ blocks which satisfies $d_1(U, W) \leq 2\delta = 2\varepsilon/3$. By the triangle inequality, we conclude that $d_1(U, \barH) \geq \Delta_\calH - \varepsilon$, as desired. Note that $M$ depends only on $\varepsilon$ and $N$, which in turn depends only on $\calH$ and $\varepsilon$.
\end{proof}

We now show how our results for orderons can be translated to finite graphs. Here we make use of several technical lemmas from~\cite{LS10}. The first lemma that we need is the following.

\begin{lemma}[Lemma 3.13(a) in~\cite{LS10}]\label{lem:upper_bound_distance_from_hered}
	For any hereditary ordered graph property $\calH$ and ordered graph $G$, we have $d_1(G, \calH) \leq d_1(W_G, \barH) \leq \Delta_{\calH}$.
\end{lemma}
While the above lemma was stated in~\cite{LS10} for hereditary properties of unordered graphs, its proof in~\cite{LS10} only uses the flexibility of a closure of a hereditary property and a simple subgraph statistics argument, and translates as-is to our ordered setting.

The next lemma that we need from~\cite{LS10} is the following.
\begin{lemma}[Lemma 2.8 in~\cite{LS10}]\label{lem:cut_norm_liminf}
	Suppose that $\|U_n - U\|_{\square} \to 0$ and $\|W_n - W\|_{\square} \to 0$ (where $U, U_n, W, W_n$ are naive orderons). Then $\liminf_{n \to \infty} d_1(W_n, U_n) \geq d_1(W, U)$.
\end{lemma}
%In our setting, we need a similar statement where the sequences converge in $d_{\triangle}$, with one of them converging to a naive block orderon). For the proof, we will first need the following lemma.

Additionally, we need the following lemma, concerning the good behavior of sequences that converge to a naive block orderon.
\begin{lemma}\label{lem:block_good_behavior}
	Fix an integer $M > 0$, and let $W$ be a naive $M$-block orderon. Also let $\{W_n\}$ be a sequence of orderons where $d_{\triangle}(W_n, W) \to 0$, and let $\{f_n\}$ be a sequence of shift functions with $\shift{f_n} \to 0$. Then it holds that $\|W_n^{f_n} - W\|_{\square} \to 0$.
\end{lemma}
\begin{proof}
	Since $d_{\triangle}(W_n, W) \to 0$, by definition of the cut-shift distance there exists a sequence $g_n$ of shift functions with $\shift{g_n} \to 0$ so that $\|W_n^{g_n} - W \|_{\square} \to 0$. By applying the shift function $h_n = f_n \circ g^{-1}_n$ to both orderons in the expression, we get that $\|W_n^{f_n} - W^{h_n}\|_\square \to 0$. On the other hand, we shall show now that $d_1(W^{h_n}, W) \to 0$. Since the cut norm is always bounded by the $L^1$-distance, we can conclude that $\|W^{h_n} - W\|_{\square} \to 0$, implying by the triangle inequality that $\|W_n^{f_n} - W\|_{\square} \to 0$.

	To show that $d_1(W^{h_n}, W) \to 0$, observe first that $\shift{h_n} \leq \shift{f_n} + \shift{g_n} \to 0$. For any pair $(x,y) \in [0,1]^2$ where both $x$ and $y$ are not $\shift{h_n}$-close to the boundary of their block (i.e., are not of the form $i/M \pm \zeta$ where $\zeta \leq \shift{h_n}$), we thus have that $W(x,y) = W^{h_n}(x,y)$. We conclude that $d_1(W^{h_n}, W)$ is bounded by the total volume of pairs $(x,y)$ that are $\shift{h_n}$-close to the boundaries, which is bounded by $4M \cdot \shift{f_n}$, and tends to zero as $n \to \infty$.
\end{proof}

Lemma~\ref{lem:upper_bound_distance_from_hered} gives us a global upper bound of $\Delta_\calH$ on the distance of any ordered graph from a hereditary property $\calH$. Our next main lemma, given below, provides an asymptotic lower bound. The statement of the lemma is analogous to (a special case of) Proposition 3.14 in~\cite{LS10}, although the proof is slightly different (and makes use of Lemma~\ref{lem:block_good_behavior}).

\begin{lemma}\label{lem:lim_inf_L1_dist}
	Let $\calP$ be any ordered graph property and let $G_n \to W$ be an ordered graph sequence that converges (in $d_{\triangle}$) to a naive block orderon. Then
	$$
	\liminf_{n \to \infty} d_1(G_n, \calP) \geq d_1(W, \barP).
	$$
\end{lemma}
\begin{proof}
	For any $n \in \mathbb{N}$ let $H_n \in \calP$ be a graph with the same size as $G_n$ satisfying $d_1(G_n, H_n) = d_1(G_n, \calP)$ (this minimum is always attained as $d_1(G_n, \calP)$ is a minimum of finitely many values). By taking a subsequence of $G_n$ for which the distance to $\calP$ converges to $\liminf d_1(G_n, \calP)$ and then taking a subsequence of it to ensure convergence of the corresponding subsequence of $H_n$, we may assume that $H_n \to U \in \barP$ (as usual, the convergence is in $d_{\triangle}$).

	By the definition of the cut-shift distance, for any $H_n$, there exists a shift function $f_n$ so that $\|W_{H_n}^{f_n} - U\|_{\square} \to 0$ and furthermore $\shift{f_n} \to 0$.
	Applying Lemma~\ref{lem:block_good_behavior} to the sequence $W_{G_n}$, which by the assumption of this lemma converges to the naive block orderon $W$, we conclude that $\|W_{G_n}^{f_n} - W\|_{\square} \to 0$. By applying Lemma~\ref{lem:cut_norm_liminf} to the sequences $W_{G_n}^{f_n}$ and $W_{H_n}^{f_n}$ which converge in cut norm to $W$ and $U$ respectively, we conclude that
	$$
	d_1(W, U) \leq \liminf_{n \to \infty} d_1(W_{G_n}^{f_n}, W_{H_n}^{f_n}) = \liminf_{n \to \infty} d_1(G_n, H_n) = \liminf_{n \to \infty} d_1(G_n, \calP),
	$$
	where the first equality follows from the fact that shifting two orderons by the same shift does not change the $L^1$-distance between them, and the second equality follows from our choice of $H_n$.
\end{proof}

We are now ready to put it all together and prove Theorem~\ref{thm:ordered_Alon_Stav}.

\begin{proofof}{Theorem~\ref{thm:ordered_Alon_Stav}}
	By Lemma~\ref{lem:upper_bound_distance_from_hered} we know that $\overline{d_\calH} \leq \Delta_{\calH}$. Thus, it suffices to show the statement of the theorem with $\overline{d_\calH}$ replaced by $\Delta_{\calH}$.
	By Lemma~\ref{lem:naive_block_orderon_far}, there exists a naive block orderon $W$, whose number of blocks $M$ is only a function of $\calH$ and $\varepsilon$, for which $d_1(W, \barH) \geq \Delta_{\calH} - \varepsilon/2$. By Lemma~\ref{lem:lim_inf_L1_dist}, there exist $\delta > 0$ and $N$ so that any ordered graph $G$ on $n \geq N$ vertices with $d_\triangle(W_{G}, W) \leq \delta$ satisfies $d_1(G, \calH) \geq d_1(W, \barH) - \varepsilon/2 \geq \Delta_{\calH} - \varepsilon$. Pick $G$ according to the random model $\bG(n, W)$. From our sampling result, Theorem~\ref{thm:Sampling}, the probability that $d_{\triangle}(W_{\bG(n, W)}, W) \leq \delta$ tends to one as $n \to \infty$. As the random model $\bG(n,W)$ is precisely a consecutive stochastic block model on $M$ blocks with parameters as in the statement of the theorem, the proof follows.
\end{proofof}
